Textureless Object Recognition: An Edge-based Approach

Textureless object recognition has become a significant task in Computer Vision with the advent of Robotics and its applications in manufacturing sector. It has been challenging to obtain good accuracy in real time because of its lack of discriminative features and reflectance properties which makes the techniques for textured object recognition insufficient for textureless objects. A lot of work has been done in the last 20 years, especially in the recent 5 years after the TLess and other textureless dataset were introduced. In this project, by applying image processing techniques we created a robust augmented dataset from initial imbalanced smaller dataset. We extracted edge features, feature combinations and RGB images enhanced with feature/feature combinations to create 15 datasets, each with a size of ~340,000. We then trained four classifiers on these 15 datasets to arrive at a conclusion as to which dataset performs the best overall and whether edge features are important for textureless objects. Based on our experiments and analysis, RGB images enhanced with combination of 3 edge features performed the best compared to all others. Model performance on dataset with HED edges performed comparatively better than other edge detectors like Canny or Prewitt.

==> untitled.tex <==
\bibitem{eggert1993scale}Eggert, D., Bowyer, K., Dyer, C., Christensen, H. \& Goldgof, D. The scale space aspect graph. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. \textbf{15}, 1114-1130 (1993)
\bibitem{steger2002occlusion}Steger, C. Occlusion, clutter, and illumination invariant object recognition. {\em International Archives Of Photogrammetry Remote Sensing And Spatial Information Sciences}. \textbf{34}, 345-350 (2002)
\bibitem{cyr2004similarity}Cyr, C. \& Kimia, B. A similarity-based aspect-graph approach to 3D object recognition. {\em International Journal Of Computer Vision}. \textbf{57}, 5-22 (2004)
\bibitem{maini2010comprehensive}Maini, R. \& Aggarwal, H. A comprehensive review of image enhancement techniques. {\em ArXiv Preprint ArXiv:1003.4053}. (2010)
\bibitem{al2010image}Al-Amri, S., Kalyankar, N. \& Khamitkar, S. Image segmentation by using edge detection. {\em International Journal On Computer Science And Engineering}. \textbf{2}, 804-807 (2010)
\bibitem{hinterstoisser2011multimodal}Hinterstoisser, S., Holzer, S., Cagniart, C., Ilic, S., Konolige, K., Navab, N. \& Lepetit, V. Multimodal templates for real-time detection of texture-less objects in heavily cluttered scenes. {\em 2011 International Conference On Computer Vision}. pp. 858-865 (2011)
\bibitem{hinterstoisser2011gradient}Hinterstoisser, S., Cagniart, C., Ilic, S., Sturm, P., Navab, N., Fua, P. \& Lepetit, V. Gradient response maps for real-time detection of textureless objects. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. \textbf{34}, 876-888 (2011)
\bibitem{ulrich2011combining}Ulrich, M., Wiedemann, C. \& Steger, C. Combining scale-space and similarity-based aspect graphs for fast 3D object recognition. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. \textbf{34}, 1902-1914 (2011)
\bibitem{tombari2013bold}Tombari, F., Franchi, A. \& Di Stefano, L. BOLD features to detect texture-less objects. {\em Proceedings Of The IEEE International Conference On Computer Vision}. pp. 1265-1272 (2013)
\bibitem{fischer2013feature}Fischer, J., Bormann, R., Arbeiter, G. \& Verl, A. A feature descriptor for texture-less object representation using 2D and 3D cues from RGB-D data. {\em 2013 IEEE International Conference On Robotics And Automation}. pp. 2112-2117 (2013)
\bibitem{bali2015review}Bali, A. \& Singh, S. A review on the strategies and techniques of image segmentation. {\em 2015 Fifth International Conference On Advanced Computing And Communication Technologies}. pp. 113-120 (2015)
\bibitem{janani2015image}Janani, P., Premaladha, J. \& Ravichandran, K. Image enhancement techniques: A study. {\em Indian Journal Of Science And Technology}. \textbf{8}, 1-12 (2015)
\bibitem{hodavn2015detection}Hodaň, T., Zabulis, X., Lourakis, M., Obdržálek, Š. \& Matas, J. Detection and fine 3D pose estimation of texture-less objects in RGB-D images. {\em 2015 IEEE/RSJ International Conference On Intelligent Robots And Systems (IROS)}. pp. 4421-4428 (2015)
\bibitem{makandar2015image}Makandar, A. \& Halalli, B. Image enhancement techniques using highpass and lowpass filters. {\em International Journal Of Computer Applications}. \textbf{109}, 12-15 (2015)
\bibitem{xie2015holistically}Xie, S. \& Tu, Z. Holistically-nested edge detection. {\em Proceedings Of The IEEE International Conference On Computer Vision}. pp. 1395-1403 (2015)
\bibitem{wang2015textured}Wang, W., Chen, L., Liu, Z., Kühnlenz, K. \& Burschka, D. Textured/textureless object recognition and pose estimation using RGB-D image. {\em Journal Of Real-Time Image Processing}. \textbf{10}, 667-682 (2015)
\bibitem{ren2015faster}Ren, S., He, K., Girshick, R. \& Sun, J. Faster r-cnn: Towards real-time object detection with region proposal networks. {\em Advances In Neural Information Processing Systems}. pp. 91-99 (2015)
\bibitem{jiang2016object}Jiang, L., Koch, A. \& Zell, A. Object recognition and tracking for indoor robots using an RGB-D sensor. {\em Intelligent Autonomous Systems 13}. pp. 859-871 (2016)
\bibitem{chan2016border}Chan, J., Addison Lee, J. \& Kemao, Q. Border: An oriented rectangles approach to texture-less object recognition. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 2855-2863 (2016)
\bibitem{wang2016self}Wang, Y. \& Deng, W. Self-restraint object recognition by model based CNN learning. {\em 2016 IEEE International Conference On Image Processing (ICIP)}. pp. 654-658 (2016)
\bibitem{verma2016vision}Verma, N., Sharma, T., Rajurkar, S., Ranjan, R. \& Salour, A. Vision based counting of texture-less objects using shape and color features. {\em 2016 11th International Conference On Industrial And Information Systems (ICIIS)}. pp. 253-258 (2016)
\bibitem{peng2016object}Peng, Y., Bao, L. \& Pi, L. Object (s)-of-interest segmentation for images with inhomogeneous intensities based on curve evolution. {\em Neurocomputing}. \textbf{195} pp. 13-18 (2016)
\bibitem{thoduka2016rgb}Thoduka, S., Pazekha, S., Moriarty, A. \& Kraetzschmar, G. RGB-D-Based Features for Recognition of Textureless Objects. {\em Robot World Cup}. pp. 294-305 (2016)
\bibitem{chan2017bind}Chan, J., Addison Lee, J. \& Kemao, Q. BIND: binary integrated net descriptors for texture-less object recognition. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 2068-2076 (2017)
\bibitem{hodan2017t}Hodan, T., Haluza, P., Obdržálek, Š., Matas, J., Lourakis, M. \& Zabulis, X. T-LESS: An RGB-D dataset for 6D pose estimation of texture-less objects. {\em 2017 IEEE Winter Conference On Applications Of Computer Vision (WACV)}. pp. 880-888 (2017)
\bibitem{bloice2017augmentor}Bloice, M., Stocker, C. \& Holzinger, A. Augmentor: an image augmentation library for machine learning. {\em ArXiv Preprint ArXiv:1708.04680}. (2017)
\bibitem{xiang2017posecnn}Xiang, Y., Schmidt, T., Narayanan, V. \& Fox, D. Posecnn: A convolutional neural network for 6d object pose estimation in cluttered scenes. {\em ArXiv Preprint ArXiv:1711.00199}. (2017)
\bibitem{jeong2018image}Jeong, H., Park, K. \& Ha, Y. Image preprocessing for efficient training of YOLO deep learning networks. {\em 2018 IEEE International Conference On Big Data And Smart Computing (BigComp)}. pp. 635-637 (2018)
\bibitem{tsai2018real}Tsai, C. \& Yu, C. Real-time textureless object detection and recognition based on an edge-based hierarchical template matching algorithm. {\em J. Appl. Sci. Eng.}. \textbf{21}, 229-240 (2018)
\bibitem{redmon2018yolov3}Redmon, J. \& Farhadi, A. Yolov3: An incremental improvement. {\em ArXiv Preprint ArXiv:1804.02767}. (2018)
\bibitem{huang2019rapid}Huang, R., Gu, J., Sun, X., Hou, Y. \& Uddin, S. A Rapid Recognition Method for Electronic Components Based on the Improved YOLO-V3 Network. {\em Electronics}. \textbf{8}, 825 (2019)
\bibitem{agustsson2019interactive}Agustsson, E., Uijlings, J. \& Ferrari, V. Interactive Full Image Segmentation by Considering All Regions Jointly. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 11622-11631 (2019)
\bibitem{fang2019dog}Fang, W., Ding, Y., Zhang, F. \& Sheng, V. DOG: A new background removal for object recognition from images. {\em Neurocomputing}. \textbf{361} pp. 85-91 (2019)
\bibitem{li2019light}Li, Y. \& Ren, F. Light-Weight RetinaNet for Object Detection. {\em ArXiv Preprint ArXiv:1905.10011}. (2019)
\bibitem{park2019multi}Park, K., Patten, T., Prankl, J. \& Vincze, M. Multi-task template matching for object detection, segmentation and pose estimation using depth images. {\em 2019 International Conference On Robotics And Automation (ICRA)}. pp. 7207-7213 (2019)
\bibitem{he2017mask}He, K., Gkioxari, G., Dollár, P. \& Girshick, R. Mask r-cnn. {\em Proceedings Of The IEEE International Conference On Computer Vision}. pp. 2961-2969 (2017)
\bibitem{yu2018fast}Yu, H., Qin, H. \& Peng, M. A Fast Approach to Texture-Less Object Detection Based on Orientation Compressing Map and Discriminative Regional Weight. {\em Algorithms}. \textbf{11}, 201 (2018)
\bibitem{xie2015holistically}Xie, S. \& Tu, Z. Holistically-nested edge detection. {\em Proceedings Of The IEEE International Conference On Computer Vision}. pp. 1395-1403 (2015)

